Porous Convection in the Discrete Exterior Calculus with Geometric Multigrid

The discrete exterior calculus (DEC) defines a family of discretized differential operators which preserve certain desirable properties from the exterior calculus. We formulate and solve the porous convection equations in the DEC via the Decapodes.jl embedded domain-specific language (eDSL) for multiphysics problems discretized via CombinatorialSpaces.jl. CombinatorialSpaces.jl is an open-source Julia library which implements the DEC over simplicial complexes, and now offers a geometric multigrid solver over maps between subdivided simplicial complexes. We demonstrate numerical results of multigrid solvers for the Poisson problem and porous convection problem, both as a standalone solver and as a preconditioner for open-source Julia iterative methods libraries.

==> csc-matrix_template.tex <==
\begin{figure}[h!]
    \centering
    \begin{asy}
        unitsize(2.1cm);

    path make_path(pair[] As) {
    	path p;
        for (pair q : As) {
        	p = p--q;
        }
        return p;
    }
    void label(string[] ses, pair[] As,pair[] Ds) {
    	for (int i = 0; i < As.length; ++i) {
          label(ses[i],As[i],Ds[i]);
        }
    }
    
    pair[] As = new pair[] {(0,0),(1/2,0),(1,0),(3/4,sqrt(3)/4),(1/2,sqrt(3)/2),(1/4,sqrt(3)/4)};
    As.append(rotate(60)*(new pair[] {As[3],As[4],As[5]}));
    As = shift((-1/3,0))*As;
    dot(As);
    
    
    string[] ses = {"$v_1$","$v_2$","$v_3$","$v_4$","$v_5$","$v_6$","$v_7$","$v_8$","$v_9$"};
    pair[] Ds = map(new pair(pair p){return 2*(p-1/3*(As[0]+As[2]+As[4]));},As);
    Ds[5] *= 2.5;
    draw(make_path(As)--cycle);
    draw(As[1]--As[3]--As[5]--cycle);
    draw(As[4]--As[6]--As[8]--As[5]--As[0]);
    label(ses,As,Ds);
    
    draw("$A$",(10/9,sqrt(3)/4)--(19/9,sqrt(3)/4),arrow=Arrow(arrowhead=TeXHead),3*N);
    
    pair[] Bs_pair = shift((3.25,0))*new pair[] {(0,0),(1,0),(1/2,sqrt(3)/2),(-1/2,sqrt(3)/2)};
    path Bs = make_path(Bs_pair);
    draw(Bs--cycle);
    draw(Bs_pair[0]--Bs_pair[2]);
    dot(Bs);
    label(new string[] {"$w_1$","$w_2$","$w_3$","$w_4$"},Bs_pair,shift(-(3,sqrt(3)/4))*Bs_pair);
    \end{asy}
    \[
    A=\begin{bmatrix} 
    1&1/2&0&0&0&1/2&0&0&1/2\\ 
    0&1/2&1&1/2&0&0&1/2&0&0\\
    0&0&0&1/2&1&1/2&1/2&0&0\\
    0&0&0&0&0&1/2&1/2&1&1/2
    \end{bmatrix}\]
    \[=\begin{bmatrix}1&.5&.5&.5&.5&1&.5&.5&.5&1&.5&.5&.5&.5&1&.5\\
    1&1&1&1&2&2&2&2&3&3&3&3&4&4&4&4\\
    0&1&3&4&6&7&10&13&14&16\end{bmatrix}
    \]
    \caption{A two-simplex subdivision, with its 
    matrix represented both densely and in the CSC 
    sparse representation we primarily utilize.}
    \label{fig:barycentric-csc}
\end{figure}

==> img/barycentric-coords_template.tex <==
\begin{asy}[inline=true]
size(12cm,0);
pair[] xs = {(0,0),(2,1),(5,0)};
string[] ns = {"$x$","$y$","$z$"};
pair[] ds = {W,N,E};

path p = scale(2)*unitcircle;
guide t;

for (int i = 0; i < 3; ++i) {
	t = t -- xs[i];
    fill(xs[i],p);
    label(ns[i],xs[i],ds[i]);
}
draw(t--cycle);

string string(real[] a) {
	string s;
    for (int i = 0; i < a.length; ++i){
    	s += string(a[i],2);
    }
    return s;
}

real[][] barys = {{1/3,1/3,1/3},{1/4,0,3/4},{5/12,1/2,1/12}};
string[] labs = {"$[\frac 13,\frac 13,\frac 13]$","$[\frac 14,0,\frac 34]$","$[\frac 5{12},\frac 12, \frac 1{12}]$"};
pair[] dss = {S,S,(2/3,1/3)};

for (int i = 0; i < barys.length; ++i){
	pair pt = barys[i][0]*xs[0]+barys[i][1]*xs[1]+barys[i][2]*xs[2];
    fill(pt,p);
    label(labs[i],pt,dss[i]);
}
\end{asy}
